Out-of-distribution detection in satellite image classification

In satellite image analysis, distributional mismatch between the training and test data may arise due to several reasons, including unseen classes in the test data and differences in the geographic area. Deep learning based models may behave in unexpected manner when subjected to test data that has such distributional shifts from the training data, also called out-of-distribution (OOD) examples. Predictive uncertainly analysis is an emerging research topic which has not been explored much in context of satellite image analysis. Towards this, we adopt a Dirichlet Prior Network based model to quantify distributional uncertainty of deep learning models for remote sensing. The approach seeks to maximize the representation gap between the in-domain and OOD examples for a better identification of unknown examples at test time. Experimental results on three exemplary test scenarios show the efficacy of the model in satellite image analysis.

==> input_files/ResultTable.tex <==
\begin{table}[!ht]
	\begin{tabular}{|l|c|c|c|}
		\hline 
						&Test Case 1 		&Test Case 2 		&Test Case 3\\ \hline 
		Max. Prob. 		&$92.34\pm0.0$			&$81.05\pm0.0$			&$83.36\pm0.0$ \\
		Mutual Info. 	&$95.34\pm0.0$			&$85.14\pm0.0$			&$89.10\pm0.0$ \\
		Entropy 		&$93.97\pm0.0$			&$82.82\pm0.0$			&$86.46\pm0.0$\\
		Log-Sum 		&$95.16\pm0.0$			&$85.11\pm0.0$			&$89.10\pm0.0$\\\hline 
	\end{tabular}
	\caption{Results of the \DPNminus on the given testing data set. Results are given as mean and standard deviation of five runs.}
\end{table}
\begin{table}[!ht]
	\begin{tabular}{|l|c|c|c|}
		\hline 
						&Test Case 1 		&Test Case 2 		&Test Case 3\\ \hline 
		Max. Prob. 		&$0.0\pm0.0$			&$0.0\pm0.0$			&$0.0\pm0.0$ \\
		Mutual Info. 	&$0.0\pm0.0$			&$0.0\pm0.0$			&$0.0\pm0.0$ \\
		Entropy 		&$0.0\pm0.0$			&$0.0\pm0.0$			&$0.0\pm0.0$\\
		Diff. Entropy 	&$0.0\pm0.0$			&$0.0\pm0.0$			&$0.0\pm0.0$\\\hline 
	\end{tabular}
	\caption{Results of the binary classifier on the given testing data set. Results are given as mean and standard deviation of five runs.}
\end{table}
\begin{table}[!ht]
	\begin{tabular}{|l|c|c|c|}
		\hline 
						&Test Case 1 		&Test Case 2 		&Test Case 3\\ \hline 
		Max. Prob. 		&$98.48\pm0.0$			&$87.60\pm0.0$	&$95.29\pm0.0$ \\
		Mutual Info. 	&$99.59\pm0.0$			&$88.52\pm0.0$	&$98.38\pm0.0$ \\
		Entropy 		&$98.94\pm0.0$			&$88.94\pm0.0$	&$96.64\pm0.0$\\
		Log-Sum 		&$99.59\pm0.0$			&$88.44\pm0.0$	&$98.46\pm0.0$\\\hline 
	\end{tabular}
	\caption{Results of the \DPNminus on the left-out 10\% of the training data set. Results are given as mean and standard deviation of five runs.}
\end{table}
\begin{table}[!ht]
	\begin{tabular}{|l|c|c|c|}
		\hline 
						&Test Case 1 		&Test Case 2 		&Test Case 3\\ \hline 
		Max. Prob. 		&$0.0\pm0.0$			&$0.0\pm0.0$			&$0.0\pm0.0$ \\
		Mutual Info. 	&$0.0\pm0.0$			&$0.0\pm0.0$			&$0.0\pm0.0$ \\
		Entropy 		&$0.0\pm0.0$			&$0.0\pm0.0$			&$0.0\pm0.0$\\
		Diff. Entropy 	&$0.0\pm0.0$			&$0.0\pm0.0$			&$0.0\pm0.0$\\\hline 
	\end{tabular}
	\caption{Results of the binary classifier on the left-out 10\% of the training data set. Results are given as mean and standard deviation of five runs.}
\end{table}

==> input_files/ResultTable_Big_save.tex <==

\begin{table*}[!ht]
	\centering
	\caption{Results of the proposed \DPNminus and a binary classifier baseline network. The table contains AUROC scores based on maximum probability, mutual information, and precision for the \DPNminus. For the binary classifier, only the maximum probability is considered, since $\alpha_0$ is related to the Dirichlet distribution and mutual information can not be applied on a single categorical distribution. The results are given as mean and standard deviation of five runs.}
	\label{tab:results}
	\begin{tabular}{|p{2cm}|l|c|c|c|c|c|c|}
		\hline & &\multicolumn{3}{|c|}{\DPNminus network}
			   &\multicolumn{3}{|c|}{Binary Classifier}\\
		\hline 
						& &Test Case 1 		&Test Case 2 		&Test Case 3
						&Test Case 1 		&Test Case 2 		&Test Case 3\\ \hline 
	\multirow{3}{2cm}{Testing Data Set}
		&Max. Prob.		&$95.51\pm1.63$			&$73.99\pm3.59$		&$81.15\pm3.46$
						&$90.67\pm1.1$			&$60.31\pm4.53$		&$53.73 \pm 9.86$\\
		&Mutual Info. 	&$96.28\pm0.57$			&$81.81\pm1.68$		&$87.03\pm1.21$ 
						&-						&-						&-	\\
						%&$85.05\pm0.0$			&$49.86\pm0.0$			&$60.37\pm0.0$\\
		%&Dif. Entropy 	&$44.14\pm0.0$			&$82.82\pm0.0$			&$86.46\pm0.0$
		%				&$0.0\pm0.0$			&$0.0\pm0.0$			&$0.0\pm0.0$\\
		&$\alpha_0$		&$96.26\pm0.51$			&$85.15\pm1.94$			&$86.94\pm1.17$
						&-						&-						&-	\\ \hline
						%&$84.78\pm0.0$			&$47.93\pm0.0$			&$60.11\pm0.0$\\\hline 

\multirow{3}{2cm}{Left out 10\% of Training Data Set}		
		&Max. Prob. 	&$98.66\pm0.37$			&$87.88\pm2.54$		&$92.27\pm2.88$ 
						&$91.87\pm1.76$			&$73.49\pm4.58$		&$0.0\pm0.0$\\
		&Mutual Info. 	&$99.24\pm0.32$			&$93.85\pm1.06$		&$95.62\pm2.80$ 
						&-						&-						&-	\\
						%&$90.57\pm0.0$			&$60.73\pm0.0$		&$75.55\pm0.0$\\
		%&Dif. Entropy	&$45.23\pm0.0$			&$88.94\pm0.0$		&$96.64\pm0.0$
		%				&$90.65\pm0.0$			&$62.33\pm0.0$		&$75.58\pm0.0$\\
		&$\alpha_0$		&$99.23\pm0.33$			&$95.01\pm0.88$		&$95.53\pm2.75$
						&-						&-						&-	\\\hline
						%&$90.35\pm0.0$			&$58.94\pm0.0$		&$75.37\pm0.0$\\\hline 
	\end{tabular}
\end{table*}

==> input_files/SimplexRepresentation.tex <==
\begin{figure}[h]
	\centering
	\subfigure[]{%
		%\label{fig:first}
		\includegraphics[height=1.4 cm]{figures/simplexVisualization/confident_sharp.png}
		\label{simplexConfident}
	}%
%	\hspace{0.3 cm}
	\subfigure[]{%
		%\label{fig:first}
		\includegraphics[height=1.4 cm]{figures/simplexVisualization/dir_10.png}
		\label{simplexDataUncertaintyIdeal}
	}%
%	\hspace{0.5 cm}
%	\subfigure[]{%
%		%\label{fig:first}
%		\includegraphics[height=1.5 cm]{figures/simplexVisualization/dir_5.png}
%		\label{simplexDataUncertaintyPractical}
%	}%
%	\\
%    \hspace{0.3cm}
	\subfigure[]{%
		%\label{fig:first}
		\includegraphics[height=1.4 cm]{figures/simplexVisualization/dir_1010.png}
		\label{simplexOODDpn}
	}%
%	\hspace{0.3 cm}
	\subfigure[]{%
		%\label{fig:first}
		\includegraphics[height=1.4 cm]{figures/simplexVisualization/dir_fraction.png}
		\label{simplexOODAfterPrecisionRegularization}
	}%\
	%\caption{Different predictive uncertainties shown over simplex: (a) In-domain confident, (b) In-domain data uncertainty (desired), (c)  In-domain data uncertainty (in practice), (d) OOD (with DPN \cite{malinin2018predictive}), and  (e) OOD (with	precision regularization)}
	\caption{Different desired predictive uncertainties shown over the simplex (cf. \cite{nandy2020towards}): (a) In-domain confident, (b) In-domain aleatoric uncertainty, (c) OOD (with DPN \cite{malinin2018predictive}), (d) OOD (with \DPNminus \cite{nandy2020towards}).}
	\label{figureSimplexRepresentation}
           \vspace{-0.5cm}
\end{figure}
